An Empirical Study on the Impact of Code Duplication-aware Refactoring Practices on Quality Metrics

Context: Code refactoring is widely recognized as an essential software engineering practice that improves the understandability and maintainability of source code. Several studies attempted to detect refactoring activities through mining software repositories, allowing one to collect, analyze, and get actionable data-driven insights about refactoring practices within software projects. Objective: Our goal is to identify, among the various quality models presented in the literature, the ones that align with the developer's vision of eliminating duplicates of code, when they explicitly mention that they refactor the code to improve them. Method: We extract a corpus of 332 refactoring commits applied and documented by developers during their daily changes from 128 open-source Java projects. In particular, we extract 32 structural metrics from which we identify code duplicate removal commits with their corresponding refactoring operations, as perceived by software engineers. Thereafter, we empirically analyze the impact of these refactoring operations on a set of common state-of-the-art design quality metrics. Results: The statistical analysis of the results obtained shows that (i) some state-of-the-art metrics are capable of capturing the developer's intention of removing code duplication; and (ii) some metrics are being more emphasized than others. We confirm that various structural metrics can effectively represent code duplication, leading to different impacts on software quality. Some metrics contribute to improvements, while others may lead to degradation. Conclusion: Most of the mapped metrics associated with the main quality attributes successfully capture developers' intentions for removing code duplicates, as is evident from the commit messages. However, certain metrics do not fully capture these intentions

==> Tables/RelatedWork.tex <==
\begin{table*}
  \centering
	 \caption{A summary of the literature on the impact of refactoring activities on software quality attributes.}
	 \label{Table:Quality Metrics in Related Work}
%\begin{sideways}
\begin{adjustbox}{width=1.0\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lllllll}\hline
\toprule
\bfseries Study & \bfseries Year & \bfseries Approach & \bfseries Software Metric & \bfseries Internal Quality Attribute   \\
\midrule
Sahraoui \etal \cite{sahraoui2000can} & 2000 & Analyzing code histories & CLD / NOC / NMO / NMI    & Inheritance / Coupling   \\ 
& & & NMA / SIX / CBO / DAC & & \\
& & & IH-ICP / OCAIC / DMMEC / OMMEC &  \\ \hline
\cellcolor{gray!30}Stroulia \& Kapoor \cite{stroulia2001metrics} & \cellcolor{gray!30}2001 & \cellcolor{gray!30}Performing a case study & \cellcolor{gray!30}LOC / LCOM / CC & \cellcolor{gray!30}Size / Coupling  \\ \hline
Fioravanti \etal \cite{fioravanti2001reengineering} & 2001 & Analyzing code histories & NL / NLID / NLIDS / IID / IID\_S & N/A \\ 
& & & NAL / NALST / TNAL / TLOC / NCL \\
& & & TNML / Nbyte / Nfile \\ \hline
\cellcolor{gray!30}Antoniol \etal \cite{antoniol2002analyzing} & \cellcolor{gray!30}2002 & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}NPS / LOC / NOS / CC / NLV & \cellcolor{gray!30}Coupling/ Size/ Complexity \\
\cellcolor{gray!30}& \cellcolor{gray!30}& \cellcolor{gray!30} & \cellcolor{gray!30}NLNV / NALO / NFC / NREP / NSPAF & \cellcolor{gray!30} \\
\cellcolor{gray!30}& \cellcolor{gray!30}& \cellcolor{gray!30}& \cellcolor{gray!30}NAA / NLK & \cellcolor{gray!30} \\ \hline
Kataoka \etal  \cite{kataoka2002quantitative} & 2002 & Analyzing code histories & Coupling measures &  Coupling   \\ \hline
\cellcolor{gray!30}Demeyer \cite{demeyer2002maintainability} & \cellcolor{gray!30}2002 & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}N/A & \cellcolor{gray!30}Polymorphism    \\ \hline
Tahvildari \etal  \cite{tahvildari2003quality} & 2003 & Analyzing code histories & LOC / CC / CMT / Halstead's efforts & Complexity    \\ \hline
\cellcolor{gray!30}Leitch \& Stroulia \cite{leitch2003assessing}& \cellcolor{gray!30}2003 & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}SLOC / No. of Procedure & \cellcolor{gray!30}Size  \\ \hline
Bois \& Mens \cite{du2003describing} & 2003 & Analyzing code histories & NOM / CC / NOC / CBO & Inheritance / Cohesion / Coupling / Size / Complexity   \\ 
& & & RFC / LCOM  \\ \hline
Rieger \etal \cite{rieger2004insights} & 2004 & Analyzing code histories & LOC / LCC / LIC / LEC / NSF / NCC / LLC & Size \\ \hline
\cellcolor{gray!30}Tahvildari \& Kontogiannis \cite{tahvildari2003metric} & \cellcolor{gray!30}2004 & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}LCOM / WMC / RFC / NOM   & \cellcolor{gray!30}Inheritance / Cohesion / Coupling / Complexity  \\ 
\cellcolor{gray!30}&\cellcolor{gray!30} & \cellcolor{gray!30}& \cellcolor{gray!30}CDE / DAC / TCC & \cellcolor{gray!30} \\ \hline
Bois \etal  \cite{du2004refactoring} & 2004 & Analyzing code histories & N/A & Cohesion / Coupling   \\ \hline
\cellcolor{gray!30}Bois \etal  \cite{du2005does} & \cellcolor{gray!30}2005 & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}N/A & \cellcolor{gray!30}N/A   \\  \hline
Geppert \etal  \cite{geppert2005refactoring} & 2005 & Performing a case study &  N/A & N/A  \\ \hline
\cellcolor{gray!30}Ratzinger et al. \cite{ratzinger2005improving} & \cellcolor{gray!30}2005 & \cellcolor{gray!30}Mining commit log & \cellcolor{gray!30}N/A &  \cellcolor{gray!30}Coupling  \\ 
\cellcolor{gray!30}& \cellcolor{gray!30} & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30} & \cellcolor{gray!30}  \\ \hline
Moser \etal  \cite{moser2006does} & 2006 & Analyzing code histories & CK / MCC / LOC   & Inheritance / Cohesion / Coupling / Complexity \\ \hline
\cellcolor{gray!30}Wilking \etal  \cite{wilking2007empirical} & \cellcolor{gray!30}2007 & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}CC / LOC  & \cellcolor{gray!30}Complexity    \\ \hline
Stroggylos \& Spinells \cite{stroggylos2007refactoring} & 2007 & Mining commit log & CK / Ca / NPM & Inheritance / Cohesion / Coupling / Complexity   \\ \hline
\cellcolor{gray!30}Moser \etal \cite{moser2007case} & \cellcolor{gray!30}2008 & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}CK / LOC / Effort (hour) & \cellcolor{gray!30}Cohesion / Coupling / Complexity  \\ \hline
Alshayeb \cite{alshayeb2009empirical} & 2009 & Analyzing code histories &  CK / LOC / FANOUT  & Inheritance / Cohesion / Coupling / Size   \\ \hline
\cellcolor{gray!30}Hegedus \etal  \cite{hegedHus2010effect} & \cellcolor{gray!30}2010 & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}CK  & \cellcolor{gray!30}Coupling / Complexity / Size \\
\cellcolor{gray!30}& \cellcolor{gray!30}& \cellcolor{gray!30}& \cellcolor{gray!30} & \cellcolor{gray!30} \\ \hline
Shatnawi \& Li \cite{shatnawi2011empirical} & 2011 & Analyzing code histories & CK / QMOOD &  Inheritance / Cohesion / Coupling / Polymorphism / Size      \\ 
& & & & Encapsulation / Composition / Abstraction / Messaging    \\ \hline
\cellcolor{gray!30}Bavota \etal  \cite{bavota2013empirical} & \cellcolor{gray!30}2013 & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}ICP / IC-CD / CCBC & \cellcolor{gray!30}Coupling \\
\cellcolor{gray!30}& \cellcolor{gray!30} & \cellcolor{gray!30}Surveying developers & \cellcolor{gray!30}& \cellcolor{gray!30}\\ \hline
Szoke \etal  \cite{szoke2014bulk} & 2014 & Mining commit log & CC / U / NOA / NII / NAni & Size / Complexity \\
& & Surveying developers & LOC / NUMPAR / NMni / NA & &  \\ \hline
\cellcolor{gray!30}Bavota \etal \cite{bavota2015experimental} & \cellcolor{gray!30}2015 & \cellcolor{gray!30}Mining commit log &  \cellcolor{gray!30}CK / LOC / NOA / NOO  &  \cellcolor{gray!30}Inheritance / Cohesion / Coupling / Size / Complexity & \\
\cellcolor{gray!30}& \cellcolor{gray!30}& \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}C3 / CCBC & \cellcolor{gray!30}\\ \hline
Cedrim \etal  \cite{cedrim2016does} & 2016 & Mining commit log & LOC / CBO / NOM / CC & Cohesion / Coupling / Complexity  \\
& & Analyzing code histories & FANOUT / FANIN & \\ \hline
\cellcolor{gray!30}Chavez \etal  \cite{chavez2017does} & \cellcolor{gray!30}2017 & \cellcolor{gray!30}Mining commit log & \cellcolor{gray!30}CBO / WMC / DIT / NOC & \cellcolor{gray!30}Inheritance / Cohesion / Coupling / Size / Complexity  \\ 
\cellcolor{gray!30}& \cellcolor{gray!30} & \cellcolor{gray!30}Analyzing code histories &\cellcolor{gray!30}LOC / LCOM2 / LCOM3 / WOC & \cellcolor{gray!30}  \\
\cellcolor{gray!30}& \cellcolor{gray!30} & \cellcolor{gray!30}& \cellcolor{gray!30}TCC / FANIN / FANOUT / CINT & \cellcolor{gray!30}  \\
\cellcolor{gray!30}& \cellcolor{gray!30} & \cellcolor{gray!30}& \cellcolor{gray!30}CDISP / CC / Evg / NPATH   &\cellcolor{gray!30} \\
\cellcolor{gray!30}& \cellcolor{gray!30} & \cellcolor{gray!30}& \cellcolor{gray!30}MaxNest / IFANIN / OR / CLOC & \cellcolor{gray!30}  \\
\cellcolor{gray!30}& \cellcolor{gray!30} & \cellcolor{gray!30}& \cellcolor{gray!30}STMTC / CDL / NIV / NIM / NOPA & \cellcolor{gray!30}  \\ \hline 
Pantiuchina \etal  \cite{pantiuchina2018improving} & 2018 & Mining commit log & LCOM / CBO / WMC / RFC  & Cohesion / Coupling / Complexity   \\
&  & Analyzing code histories &  C3 / B\&W / SRead  \\ \hline
%\cellcolor{gray!30}Fakhoury \etal \cite{fakhoury2019improving}    & \cellcolor{gray!30}2019 &  \cellcolor{gray!30}Mining commit log & \cellcolor{gray!30}B\&W / Sread / Dorn &   \cellcolor{gray!30}N/A \\ \cellcolor{gray!30}  &\cellcolor{gray!30}  & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30} & \cellcolor{gray!30}   \\ \hline                                   
\cellcolor{gray!30}AlOmar \etal \cite{alomar2019impact}      & \cellcolor{gray!30}2019 &  \cellcolor{gray!30}Mining commit log & \cellcolor{gray!30}LCOM / CBO / FANIN / FANOUT & \cellcolor{gray!30}Coupling / Cohesion / Complexity / Inheritance / Size  \\                                                                   \cellcolor{gray!30}    & \cellcolor{gray!30} & \cellcolor{gray!30}Analyzing code histories &  \cellcolor{gray!30}RFC / CC / WMC / Evg / NPATH & \cellcolor{gray!30}Polymorphism / Encapsulation / Abstraction   \\                                  
\cellcolor{gray!30} & \cellcolor{gray!30} &\cellcolor{gray!30} &  \cellcolor{gray!30}MaxNest / DIT / NOC / IFANIN / LOC & \cellcolor{gray!30} \\
\cellcolor{gray!30}& \cellcolor{gray!30}&\cellcolor{gray!30} &   \cellcolor{gray!30}STMTC / CDL / NIV / NIM / CLOC & \cellcolor{gray!30} \\ \hline
Pantiuchina \etal \cite{pantiuchina2020developers} & 2020 & Mining commit log & 42 product \& process metrics & Coupling / Cohesion / Complexity / Inheritance / Size \\
& & Analyzing code histories \\

%\cellcolor{gray!30}AlOmar \etal \cite{alomar2020developers}    & \cellcolor{gray!30}2020 &  \cellcolor{gray!30}Mining commit log &  \cellcolor{gray!30}LCOM / CBO / RFC / CC & \cellcolor{gray!30}Coupling / Cohesion / Complexity / Inheritance / Size \\ 
%\cellcolor{gray!30} & \cellcolor{gray!30} & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}WMC / LOC / DIT / NOC & \cellcolor{gray!30} \\ \hline
%AlOmar \etal \cite{alomar2022refactoring}    & 2021 &  Mining commit log & LCOM / CBO / FANIN / FANOUT & Coupling / Cohesion / Complexity / Inheritance / Size \\ 
%&  & Analyzing code histories & RFC / CC / WMC / NPATH &  \\
%& & &  MaxNest / DIT / NOC / IFANIN / LOC \\
%& & &   STMTC / CDL / NIV / NIM / CLOC \\ \hline
%\cellcolor{gray!30}Hamdi \etal \cite{hamdi2021empirical}    & \cellcolor{gray!30}2021 &  \cellcolor{gray!30}Mining commit log & \cellcolor{gray!30}LCOM / CBO / NOSI / TCC / LOC & \cellcolor{gray!30}Coupling / Cohesion / Complexity / Inheritance / Size \\ 
%\cellcolor{gray!30}& \cellcolor{gray!30} & \cellcolor{gray!30}Analyzing code histories & \cellcolor{gray!30}RFC / LCC / WMC / VQYT / DIT & \cellcolor{gray!30} \\ \hline
%Ouni \etal \cite{ouni2023impact}    & 2023 &  Mining commit log & LCOM / CBO / NOSI / TCC / NIV / IFANIN& Coupling / Cohesion / Complexity / Inheritance / Size \\ 
%&  & Analyzing code histories & RFC / FANIN / WMC / VQYT / NIM &  \\
%&  &  & FANOUT / CC / Evg / MaxNest / DIT &  \\
%& & &  LOC / BLOC / CLOC / STMTC / NOC & \\
\bottomrule
\end{tabular}
\end{adjustbox}
%\end{sideways}
\end{table*}
